Computational Approaches to the Detection of Lesser-Known Rhetorical Figures: A Systematic Survey and Research Challenges

Rhetorical figures play a major role in our everyday communication as they make text more interesting, more memorable, or more persuasive. Therefore, it is important to computationally detect rhetorical figures to fully understand the meaning of a text. We provide a comprehensive overview of computational approaches to lesser-known rhetorical figures. We explore the linguistic and computational perspectives on rhetorical figures, emphasizing their significance for the domain of Natural Language Processing. We present different figures in detail, delving into datasets, definitions, rhetorical functions, and detection approaches. We identified challenges such as dataset scarcity, language limitations, and reliance on rule-based methods.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> main.tex <==
% \documentclass{sig-alternate-05-2015}

% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}
% \usepackage{glossaries}
% \setlength{\marginparwidth}{2cm}
% \usepackage{todonotes}

% \input{glossary}

% \begin{document}

% % Copyright
% \setcopyright{acmcopyright}
% %\setcopyright{acmlicensed}
% %\setcopyright{rightsretained}
% %\setcopyright{usgov}
% %\setcopyright{usgovmixed}
% %\setcopyright{cagov}
% %\setcopyright{cagovmixed}


% % DOI
% %\doi{10.475/123_4}

% % ISBN
% %\isbn{123-4567-24-567/08/06}

% %Conference
% \conferenceinfo{Big Conference '16}{October 26--28, 2016, Place, Country}

% %\acmPrice{\$15.00}

% %
% % --- Author Metadata here ---
% %\conferenceinfo{WOODSTOCK}{'97 El Paso, Texas USA}
% %\CopyrightYear{2007} % Allows default copyright year (20XX) to be over-ridden - IF NEED BE.
% %\crdata{0-12345-67-8/90/01}  % Allows default copyright data (0-89791-88-6/97/05) to be over-ridden - IF NEED BE.
% % --- End of Author Metadata ---

% \title{Computational Rhetoric \\ Subtitle}

% %
% % You need the command \numberofauthors to handle the 'placement
% % and alignment' of the authors beneath the title.
% %
% % For aesthetic reasons, we recommend 'three authors at a time'
% % i.e. three 'name/affiliation blocks' be placed beneath the title.
% %
% % NOTE: You are NOT restricted in how many 'rows' of
% % "name/affiliations" may appear. We just ask that you restrict
% % the number of 'columns' to three.
% %
% % Because of the available 'opening page real-estate'
% % we ask you to refrain from putting more than six authors
% % (two rows with three columns) beneath the article title.
% % More than six makes the first-page appear very cluttered indeed.
% %
% % Use the \alignauthor commands to handle the names
% % and affiliations for an 'aesthetic maximum' of six authors.
% % Add names, affiliations, addresses for
% % the seventh etc. author(s) as the argument for the
% % \additionalauthors command.
% % These 'additional authors' will be output/set for you
% % without further effort on your part as the last section in
% % the body of your article BEFORE References or any Appendices.

% \numberofauthors{1}
% \author{
% \alignauthor
% % Author list currently alphabetical. Let's discuss this at some point.
% Ramona K\"uhn, Jelena Mitrović\\
% 	\affaddr{University of Passau}\\
% 	\affaddr{Faculty for Computer Science and Mathematics}\\
%       \affaddr{Innstra\ss{}e 43, 94032 Passau, Germany}\\
%       \email{\{ramona.kuehn,jelena.mitrovic\}@uni.passau.de}
% % 2nd. author
% %\alignauthor
% %G.K.M. Tobin\titlenote{The secretary disavows
% %any knowledge of this author's actions.}\\
% %       \affaddr{Institute for Clarity in Documentation}\\
% %       \affaddr{P.O. Box 1212}\\
% %       \affaddr{Dublin, Ohio 43017-6221}\\
% %       \email{webmaster@marysville-ohio.com}
% %% 3rd. author
% %\alignauthor Lars Th{\o}rv{\"a}ld\titlenote{This author is the
% %one who did all the really hard work.}\\
% %       \affaddr{The Th{\o}rv{\"a}ld Group}\\
% %       \affaddr{1 Th{\o}rv{\"a}ld Circle}\\
% %       \affaddr{Hekla, Iceland}\\
% %       \email{larst@affiliation.org}
% %\and  % use '\and' if you need 'another row' of author names
% %% 4th. author
% %\alignauthor Lawrence P. Leipuner\\
% %       \affaddr{Brookhaven Laboratories}\\
% %       \affaddr{Brookhaven National Lab}\\
% %       \affaddr{P.O. Box 5000}\\
% %       \email{lleipuner@researchlabs.org}
% }
% \date{\today}

% \maketitle

% \input{01_abstract}

% %
% % The code below should be generated by the tool at
% % http://dl.acm.org/ccs.cfm
% % Please copy and paste the code instead of the example below. 
% %
% %\begin{CCSXML}
% %<ccs2012>
% % <concept>
% %  <concept_id>10010520.10010553.10010562</concept_id>
% %  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
% %  <concept_significance>500</concept_significance>
% % </concept>
% % <concept>
% %  <concept_id>10010520.10010575.10010755</concept_id>
% %  <concept_desc>Computer systems organization~Redundancy</concept_desc>
% %  <concept_significance>300</concept_significance>
% % </concept>
% % <concept>
% %  <concept_id>10010520.10010553.10010554</concept_id>
% %  <concept_desc>Computer systems organization~Robotics</concept_desc>
% %  <concept_significance>100</concept_significance>
% % </concept>
% % <concept>
% %  <concept_id>10003033.10003083.10003095</concept_id>
% %  <concept_desc>Networks~Network reliability</concept_desc>
% %  <concept_significance>100</concept_significance>
% % </concept>
% %</ccs2012>  
% %\end{CCSXML}
% %
% %\ccsdesc[500]{Computer systems organization~Embedded systems}
% %\ccsdesc[300]{Computer systems organization~Redundancy}
% %\ccsdesc{Computer systems organization~Robotics}
% %\ccsdesc[100]{Networks~Network reliability}


% %
% % End generated code
% %

% %
% %  Use this command to print the description
% %
% \printccsdesc

% % We no longer use \terms command
% %\terms{Theory}

% \keywords{Fancy keywords here}

% \input{02_intro}
% \input{03_relwork}
% \input{04_modeling}
% \input{05_metaphor}
% \input{06_concl}
% \input{stuff}
% %ACKNOWLEDGMENTS are optional
% \input{07_ack}

% \bibliographystyle{abbrv}
% \bibliography{08_references}
% %\clearpage
% %\input{stuff}
% \end{document}


==> tex/03_ontologies.tex <==
\subsection{Ontologies: Formal Representations of Rhetorical Figures}
\label{subsec:ontologies}
For computational processing of rhetorical figures, unified definitions, and clear machine-readable structures and formats are necessary. In the area of rhetorical figures, this task is especially difficult as their linguistic definitions are not coherent and even differ between languages, as we have described in Section~\ref{sec:lingview}. Ontologies can help to put an end to ``inconsistent description'' and ``ambiguous term definitions'' that arise from different sources~\cite{hu2006natural}. These ontologies are formal representations of knowledge in a ``declarative and computable form''~\cite{pease2011ontology}. In the following, we give a short overview of the most important ontologies in the domain of rhetorical figures.



% An ontology consists of classes, properties, and individuals connected through relations. A domain ontology represents elements from a specific area or domain. Ontologies are established in various domains: For example, in the medical domain, they tackle ``inconsistent description'' and ``ambiguous term definitions'' that arise from different sources~\cite{hu2006natural}. The same applies to the domain of rhetorical figures, as over the centuries, different authors have tried to define rhetorical figures and find a classification scheme~\cite{quintilian1996institutio,peacham1971garden,lausberg1990handbuch}.




% Formal models are necessary to put an end to the inconsistencies and make the data machine-readable through some form of standardization.
% In domains with many varying definitions, formal models can help in the following ways~\cite{hendler2020semantic}:
% \begin{itemize}
%     \item Models support people's communication.
%     \item Models can explain and make predictions.
%     \item Models can represent commonalities and differences among multiple viewpoints.
% \end{itemize}

% The shift from informal models and descriptions of rhetorical figures to a formal representation was realized with ontologies. ``An ontology is a formal, explicit specification of a shared conceptualization'' where a conceptualization is a simplified representation of the world \cite{gruber1995toward}. Furthermore, ontologies are a formal representation of knowledge in a ``declarative and computable form''~\cite{pease2011ontology}.
% In other words, an ontology is a formal description of knowledge, forming a knowledge graph. The nodes are connected by logical relationships, allowing to model complex interrelations. It is important to connect data, as ``disconnected data result in dumb behaviour''~\cite{ALLEMANG20111}. Ontologies are structured in triples with subject, predicate, and object. Those ontologies have a defined syntax and keywords and can be queried by the query language SPARQL.



% \todo[inline]{TODO nice related work: http://ceur-ws.org/Vol-2969/paper42-CAOS.pdf}


One of the first approaches towards a formal description of rhetorical figures was presented by Harris and Di Marco~\cite{harris2009constructing} in 2009 in their \textbf{Rhetorical Figuration Ontology}. They theoretically describe how such an ontology could look like. They focus on linguistic operations of rhetorical figures such as addition, deletion, permutation, and cognitive affinities (e.g., comparison, contrast, symmetry). The authors, however, remark that their approach does not work for structures with homonyms, i.e., same words with different meanings, or the same word in a different form (e.g., because of inflection).

% Multiple ontologies were developed by O'Reilly and Paurobally~\cite{o2010lassoing} for the \textbf{LaRhetO} application. With them, they try to discover rhetorical forms in natural language. OWL, SWRL, the semantic web, and linked data are used to describe rhetorical figures. However, the authors remark that it is not possible to describe all rhetorical figures with ``simple logic rules''. 

The project \textbf{RhetFig} from Kelly et al.~\cite{kelly2010toward} had the goal of building a database, a wiki, and an ontology for rhetorical figures of speech. The authors developed an advanced set of relations to overcome limitations from previous research.
They classified rhetorical figures into the three groups called tropes (figurative usage and conceptual similarities e.g., metaphor, irony), schemes (formal figures based on a certain syntax or structure)
% e.g., alliteration: ``\textit{t}he  \textit{t}errible \textit{t}iger'')
, and chroma (a figure used intentionally). In addition, they assigned linguistic domains to the figures, e.g., phonological, or morphological. 
 
While previous models were rather directed towards the English language, Mladenović and Mitrović~\cite{mladenovic} transferred the concepts successfully to the Serbian language and built an ontology of 98 Serbian rhetorical figures. This ontology is called \textbf{RetFig} (without the letter ``h'') and was modeled in OWL. 

% A model of an ontology with a focus on cognitive aspects and relations between rhetorical figures was presented by Harris et al.~\cite{harris2017cognitive} in their \textbf{cognitive ontology}. They present  three methodologies(top down, middle out, and bottom up) for building ontologies of rhetorical figures. Especially, they highlight the form-function correlation and cognitive effects of each figure. They describe the phenomenon of lexical priming that certain words trigger the recall of other words that are semantically, phonologically, or morphologically close (e.g., ``key'' triggers ``lock'', ``door'', ``cue'', ``keystone''). Also, it is mentioned that it is known that figures with repetition are more memorable than others.

% A survey of ontological modeling of rhetorical concepts is described by \cite{mitrovic2017ontological}. They compare the Rhetorical Structure Theory (RST), the Serbian RetFig ontology, and the Lassoing Rhetoric project~\cite{o2010lassoing}.


% The \textbf{Antimetabole Ontology} -- an ontology especially for the figure antimetabole -- is presented by O'Reilly and Harris~\cite{o2017antimetabole}. Their ontology also contains a description of force vectors that model the figure. However, they state that this model can be applied to other balanced figures such as anadiplosis, parallelism, and epanalepsis.



% The \textbf{Climax Ontology} for the rhetorical figures anadiplosis, incrementum, gradatio, and climax is presented by O'Reilly et al.~\cite{o2018arguments}. Its structure is based on the RetFig ontology by Harris et al.~\cite{harris2017cognitive}. The ontology itself is written in OWL and evaluated with SPARQL queries.


% % Recent research focuses to model figures in the English language. Often, only a few rhetorical figures are modeled, but then in detail. E.g. modeling chiasmus, epanaphora, epiphora~\cite{dubremetz2018rhetorical}, or gradatio, incrementum and climax~\cite{o2018arguments}) similar to black

% An \textbf{extended Climax Ontology} is presented by Black et al.~\cite{black2019ontological}. The authors of this research actually overlap significantly with those from the Climax ontology~\cite{o2018arguments}. However, they ``underspecified'' the ontology on purpose, ``until more computational work is required''. This shows that the focus of many rhetorical ontologies often lies in formalization, while the computational part is neglected.


% That rhetorical figures are present and relevant in every domain, shows the work of Alliheedi et al.~\cite{alliheedi2019ontological}. They created a prototype \textbf{ontology for rhetorical move analysis} with a focus on arguments in the domain of biochemistry. 

% A cognitive \textbf{Litotes Ontology} was developed by Mitrović et al.~\cite{mitrovic2020cognitive}. They formally described the figure and its implications that result from the double negation. The ontology is written in OWL. They also state that their ontology is deliberately underspecified to allow a mapping onto other ontologies. Computational applications are considered future work. 

% Based on the original RetFig ontology~\cite{harris2009constructing}, Wang et al.~\cite{wang2021ontology} developed an ontology for figures of perfect lexical repetition, called \textbf{Ploke Ontology}. They also consider cognitive affinities in their model.

The structure of the Serbian RhetFig ontology (which is actually based on the RetFig ontology~\cite{harris2009constructing}) was reused for the formal description of 110 rhetorical figures in the \textbf{GRhOOT Ontology}~\cite{kuhn2022grhoot}.

A combination of the English Ploke, the Serbian RetFig, and the German GRhOOT ontology was presented in the \textbf{Multilingual Ontology}~\cite{wang2022towards}, describing figures of repetition in a multilingual context. This ontology benefitsl from the formal descriptions of RetFig and GRhOOT, and the cognitive affinities from the Ploke ontology.


% An overview of how the RetFig, RhetFig, Ploke, GRhOOT, and the Multilingual ontology are connected is shown by Kühn and Mitrović~\cite{kuhnmultilingual}. However, as our overview of different ontologies has shown, there are many more connections between the different ontologies. Most of them are actually based on the theoretical descriptions by Harris and Di Marco~\cite{harris2009constructing}.


% The \textbf{ESTHER ontology} is the English adaption of the GRhOOT ontology. It shares the same structure, but additionally models hierarchical and compound figures mentioned by \cite{harris2017cognitive} and \cite{o2018arguments}, \cite{black2019ontological}.



% The ontologies mentioned above are illustrated in Fig.~\ref{fig:onto_timeline} according to the year they were published. This figure clarifies their development over time (and the advances from one to the other ontology.)


% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=\textwidth]{figs/Timeline.PNG}
%     \caption{Evolution of different rhetorical ontologies\todo[inline]{update in the end with numbers}}
%     \label{fig:onto_timeline}
% \end{figure}

% \todo[inline]{remove in the end, only for figure}
% \begin{itemize}
%     \item[2009] Rhetorical Figuration Ontology, Harris and Di Marco~\cite{harris2009constructing}
%     \item[2010] RhetFig, Kelly et al.\cite{kelly2010toward}
%     \item[2010] LaRhetO, O'Reilly and Paurobally~\cite{o2010lassoing}
%     \item[2013] Serbian RetFig, Mladenović and Mitrović \cite{mladenovic}
%     \item[2017] Cognitive Ontology, Harris et al. ~\cite{harris2017cognitive}
%     \item[2017] Antimetabole ontology, O'Reilly and Harris \cite{o2017antimetabole}
%     \item[2018] Climax ontology, O'Reilly \cite{o2018arguments}
%     \item[2019] Extended climax ontoloy, Black et al.\cite{black2019ontological}
%     \item[2019] Rhetorical move ontology Alliheedi \cite{alliheedi2019ontological}
%     \item[2020] Litotes ontology, Mitrović et al.\cite{mitrovic2020cognitive} 
%     \item[2021] Ploke ontology, Wang et al.~\cite{wang2021ontology}
%     \item[2022] GRhOOT  ontology, Kühn et al.~\cite{kuhn2022grhoot}
%     \item[2022] Multilingual Ontology, Wang et al.~\cite{wang2022towards} 
%     \item[2023] ESTHER English ontology, Kühn et al.\todo[inline]{FOIS cite}
% \end{itemize}

==> tex/03_relwork.tex <==
\section{Related Work}
\label{sec:relwork}

% Do we need a related work? Because the whole paper is related work?
Other surveys of rhetorical figures in the context of NLP focus mainly on the figure metaphor. It is a figure that occurs quite often and is used in our everyday communication. Therefore, the availability of data is higher than for other figures. 

Surveys in the area of rhetorical figures in NLP only investigate the figure metaphor. It seems to be one of the most popular rhetorical figures in the context of NLP. In the survey of Shutova~\cite{shutova2010models}, they divide the automatic processing of metaphor into two tasks, namely metaphor recognition and metaphor interpretation. Recognition means to identify if a phrase has a metaphorical meaning, whereas identification means to identify the literal meaning of the metaphor.
%Our steps described in Section~\ref{sec:intro} are based on this definition. 
The survey describes different models of metaphors, problems when annotating metaphors, and gives an overview of datasets of metaphors. Most of the work mentioned relys on hand-coded knowledge. Shutova herself criticizes that although the approaches are still ``highly influential'', they will be replaced by statistical methods. She also demands a large dataset of metaphors to foster research in this direction, also with AI models.



% Kind of a survey

% 3. Automatic Metaphor recognition
% different approaches identified (sources see paper)
% \begin{itemize}
% 	\item Using hand-coded patterns (Container for content etc.)
% 	\item based on lexical patterns indicating a metaphorical expression like ``metaphorical speaking'', ``utterly'', ``literally''
% 	\item WordNet hierarchy, words that share a set of common word forms among their descendants (e.g. publication, publisher); are often metonymic
% 	\item Source-target-mapping 
% 	\item sentence clustering approach for non-literal language recognition; classification in literal and non-literal
% 	\item Literal vs. metaphorical use with maximum entropy classifier
% 	\item most of those approaches only consider metaphorical verbs, but some also noun-is-a-nount metaphor

% \end{itemize}




The survey of Rai and Chakraverty~\cite{rai2020survey} also investigates the computational processing of metaphors. They also investigate different approaches for the two subtasks of detection (called recognition by Shutova) and interpretation. They present theoretical background and different types of metaphors. In addition, they describe the computational techniques to approach the detection and identification of metaphors. Compared to the survey of Shutova, they also describe approaches based on deep learning, such as neural networks.


The survey of Ge et al.~\cite{ge2023survey} highlights the relevance of metaphors for NLP tasks such as machine translation and sentiment analysis. They consider related work under the aspects of metaphor identification, interpretation, generation, and application. According to those four categories, they present current metaphor datasets and approaches to solve the problem of each category. Compared to the other surveys before, also BERT and other language model-based approaches are presented.
We will explicitly exclude the figure metaphor from our survey as there exists already a lot of research in this field. The interested reader can however look into the above-mentioned resources for more information about metaphors.


The identification and classification of rhetorical figures have long been a focus of NLP research. However, existing studies have predominantly focused on figure detection, neglecting the subsequent analysis of their purpose and effect. Harris et al. \todo[inline]{cite} This oversight limits our understanding of the broader communicative intent and impact of rhetorical figures in NLP. We therefore encourage to follow all three steps of figure detection, identification, and interpretation we mention in Section~\ref{subsec:comprec}.


==> tex/compRhet.tex <==

\subsubsection{Computational Rhetoric and Rhetorical NLP}
\label{subsec:comprec}
mentioned by Zhan und Wan~\cite{zhang2021mover}  Figurative Language Processing (FLP) -- is this a thing? Yes it is, but rather how humans process figurative language


Rhetorical figures are necessarily linked with rhetoric. In the context of rhetorical figures in NLP, the term ``Computational Rhetoric'' is mentioned sometimes. However, as with most rhetorical figures, it has never been clearly defined. We want to investigate the literature and compare different notions of this term. 
We first investigated the ACL Anthology\footnote{https://aclanthology.org}, which is a collection of publications from major NLP conferences, journals, and workshops. The search for the literal appearance of ``Computational Rhetoric''\footnote{Link to the results: \url{https://aclanthology.org/search/?q=\%22computational+rhetoric\%22}} led to a total of two distinct results, one from 1993 and one from 2011. None of them define the term computational rhetoric. In the one of 1993, only an article with the term is cited. Therefore, we continue our search on Google Scholar. The search for the literal term ``Computational Rhetoric''\footnote{Link to the results: 
\url{https://scholar.google.com/scholar?start=0\&q=\%22computational+rhetoric\%22\&hl=de\&as_sdt=0,5}
} results in about 168 articles.

The first mention of the term in a publication in Google Scholar is in the year 1987 in the context of personal relationships. However, the paper does not contain any further explanations.


Figure~\ref{fig:numberofCompRhetPapers} shows the number of publications mentioning the term over time. "Computational Rhetoric" had its peak so far in the year 2019 with 24 publications mentioning it.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figs/NumberOfCompRhetPapers.PNG}
    \caption{Number of mentions of "Computational Rhetoric" in papers}
    \label{fig:numberofCompRhetPapers}
\end{figure}


% nach Jahren sortiert, not every paper has a year
% Jahr, Anzahl Paper
% 2023 6 
% 2022 9 
% 2021 12
% 2020 16
% 2019 24
% 2018 10
% 2017 16 
% 2016 10
% 2015 4
% 2014 3
% 2013 4
% 2012 6
% 2011 5
% 2010 7
% 2009 1
% 2008 1
% 2007 2
% 2006 2
% 2005 3
% 2004 2
% 2003 0
% 2002 3 Grasso
% 2001 0
% 2000 0
% 1999 2
% 1998 0
% 1997 0
% 1996 0
% 1995 2
% 1994 3
% 1993 4
% 1992 1
% 1991 0
% 1990 0
% 1989 0
% 1988 0
% 1987 1
% 1986 0


We use Harzing's Publish or Perish software for our purpose to display and sort the results from Google Scholar. We identify the top researchers in the domain of Computational Rhetoric. We can either rank the publications by their number of citations or use the Google Scholar rank, which is not further specified how it is calculated.

The top 25 most cited papers containing the term ``Computational Rhetoric'' are shown in Figure~\ref{fig:mostcited}.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/publishPerish.png}
    \caption{The 25 most cited publications containing ``Computational Rhetoric'' (Screenshot from Harzings Publish or Perish software).}
    \label{fig:mostcited}
\end{figure}

The top 25 publications ranked by Google Scholar are shown in Figure~\ref{fig:bestranked}.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/bestRanked.PNG}
    \caption{The 25 best-ranked publications containing ``Computational Rhetoric'' (Screenshot from Harzing's Publish or Perish software).}
    \label{fig:bestranked}
\end{figure}






We further identified the top ten researchers out of all 168 publications on Google Scholar. We only consider the first three to four researchers of a paper, as the other are truncated by the Publish or Perish software.

\begin{table}
    \centering
    \begin{tabular}{lr}
         Researcher& Number of Publications\\ \hline
         Randy Harris& 13\\
         Chrysanne DiMarco& 10\\
         Ryan Omizo& 10\\ 
         O'Reilly & 6 \\
        Jelena Mitrović & 5 \\
         Yetian Wang & 5 \\
         Michael W Wojcik & 5 \\ 
         S. Scott Graham  &    4 \\
         William Hart-Davidson   &    4 \\
         Floriana Grasso  & 4 \\ \hline
    \end{tabular}
    \caption{Top ten researchers in the area of computational rhetoric.}
    \label{tab:topResearchers}
\end{table}
Some of those authors co-authored papers together, such as Harris, DiMarco, O'Reilly, Mitrović, and Wang.



The most relevant paper  (33 citation) is from Grasso \cite{grasso2002towards} from the year 2002. Although the title is ``Towards Computational Rhetoric'', this term is not used at all in the paper itself. However, it describes the ``considerations of the communicative dimension of rhetorical argumentation'' as well as rhetoric and its applications in artificial intelligence.



\hl{Hier weitermachen}



% Top three important researcher ranked by citations
% DiMarco 4 publications
% Harris 3 publications
% Grasso 2

% Top three important researcher ranked by Google scholar rank
% Mitrović 4
% Handschuh 3
% Harris 2


% 382: https://journals.sagepub.com/doi/abs/10.1177/1461445606064836

% 193: https://library.oapen.org/handle/20.500.12657/24037


% 154: https://books.google.com/books?hl=de&lr=&id=tMuIAgAAQBAJ&oi=fnd&pg=PP1&dq=%22computational+rhetoric%22&ots=agB5atLhIq&sig=-faDYZFNLgGpKMAUyTTxReVyVbY

% 128: https://cdn.aaai.org/Symposia/Spring/1993/SS-93-02/SS93-02-025.pdf

% 100. https://library.oapen.org/handle/20.500.12657/24040

% 85: https://www.sciencedirect.com/science/article/pii/S0378720617309229

% 80: https://aclanthology.org/J93-3002.pdf

% 75: https://www.sciencedirect.com/science/article/pii/S0388000104000567



% 71: https://onlinelibrary.wiley.com/doi/abs/10.1002/int.20187

% 58: https://www.sciencedirect.com/science/article/pii/S875546151530013X

% 50: https://www.jstor.org/stable/2214213







% 43: https://books.google.com/books?hl=de&lr=&id=bkbBZcR7DG4C&oi=fnd&pg=PR7&dq=%22computational+rhetoric%22&ots=lmCJXNPLAZ&sig=j1FygHgCAEXgC1rjGdR-cTWhYwc


% 41: https://ris.utwente.nl/ws/portalfiles/portal/102041208/PersuasiveTechProceedings.pdf#page=48

% 35: https://content.iospress.com/articles/argument-and-computation/aac027

% 33: https://ojs.uwindsor.ca/ojs/leddy/index.php/informal_logic/article/view/2589


% 30: https://scholar.archive.org/work/m4gibmnas5grvf4cwqqsh2m654/access/wayback/http://pdfs.semanticscholar.org/4e84/5a8ffebbe30b6255b774bf90e536584a957b.pdf

% 29: https://content.iospress.com/articles/argument-and-computation/aac026

% 26: https://www.sciencedirect.com/science/article/pii/0167923694900345

% 23: https://link.springer.com/article/10.1007/s00146-004-0313-2
% 23: https://link.springer.com/article/10.1007/s10846-008-9228-3




% https://onlinelibrary.wiley.com/doi/epdf/10.1002/int.20187












Following with 18 citations is ``A computational approach to assessing rhetorical effectiveness'' \cite{majdik2019computational}. 




Wojcik claims that computational rhetoric means ``applying the ideas and goals of rhetoric to text processing and related areas''.\cite{wojcik2013inventing}

%q=%22computational+rhetoric%22\&hl=de\&as_sdt=0,5}} (including the quotation marks for exact word match), the search engine finds 165 results. 





% What computational rhetoric is about




Computational rhetoric connects different research areas such as computer science, rhetoric, psychology, information science, etc.~\cite{mitrovic2020cognitive}. As language is complex, the expertise from different fields can contribute to a better understanding from different perspectives as the approaches are manifold and can symbiotically profit from each other.


\cite{lawrence2017harnessing} describes the term computational rhetoric \todo[inline]{todo, grasso und co.} 
% https://scholar.google.com/scholar?start=0&q=%22computational+rhetoric%22&hl=de&as_sdt=0,5









% There exist different categories of figures: Figures of construction often contain a repetition or an omission. It is an easy task for a computer to detect repeating elements. However, it is difficult to decide, if the repetition was coincidental or used to create a rhetorical figure~\cite{dubremetz2018rhetorical}.
% It becomes even harder for rhetorical figures with a transferred meaning, where the source and target domain do not seem to be connected in any way, e.g., in the metaphor ``You are not the brightest candle on the cake'', one must see the connection between the brightness of a candle and the smartness of a person.


The term computational rhetoric seems to be too broad and encompasses much more aspects of rhetoric than only rhetorical figures. Therefore, we introduce the new field of research that we would like to call rhetorical figure NLP computation.

This describes the computational approach to rhetorical figures. We also identified different steps necessary to approach rhetorical figures from a computational perspective. 
Other researchers so far only focus on one step to label rhetorical figures, such as Zhu et al.~\cite{zhu2022configure}. They either tried figure extraction (extracting figurative units as ``smallest continuous clause sequence carrying a complete expression of
a specific figure'' where clauses are text spans that are separated by punctuation.), figure type classification (scheme or trope), or figure recognition (based on heuristic rules that search for ``obvious patterns'' such as special words ``as'', or ``like'' for metaphors or similes). 
We see some of those tasks as critical. First, they assume that a figure appears only in a part of the sentence and does not span over a whole sentence. From our point of view, this assumption holds for most of the figures. However, there are still figures that can span over a complete sentence or even across multiple consecutive sentences (e.g., anaphora, epiphora, alliteration, etc.). During the figure type classification, the authors identify if the found figure belongs to the category ``trope'' or ``scheme''. We are unsure to what extent that helps find the actual figure or its purpose. In addition, they investigate only 12 figures. Furthermore, they rely on special words to identify figures, but a metaphor does not necessarily contain the mentioned words. 





Considering the taxonomy of fields of studies in NLP in Figure\ref{fig:nlptaxonomy}, we realize how many fields are affected by rhetorical figures. The authors Schopf et al.~\cite{schopf2023exploring} defined 12 fields of studies in NLP, each with subfields. Please note that those fields often cannot be considered separately as there are often intersections with other fields. The authors of the taxonomy also mention this issue. However, when considering in which fields rhetorical figures can be involved, this intersection of fields becomes even more obvious. We adapted the figure and highlighted the fields in which rhetorical figures play a role.

\cite{zhu2021self} also state that figure detection (in their specific case: euphemism detection) is related to sense discovery of unknown words and word sense disambiguation.




\todo[inline]{build figure, add category Computational Rhetoric, and highlight subcategories}.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/NLPtaxonomy.png}
    \caption{Taxonomy of fields of study in NLP, own illustration adapted from Schopf et al. \cite{schopf2023exploring}. Highlighted are the fields that play a role in the computational processing of rhetorical figures. Furthermore, we added the field ``Computational Rhetoric'' in the section of Linguistics \& Cognitive NLP.\hl{Adapt figure}.}
    \label{fig:nlptaxonomy}
\end{figure}
As shown, the topic of rhetorical figures is an intersection of other categories in NLP. However, it is also considered to be an own research direction as it is a complex field. It is often referred to as ``Computational Rhetoric''. We placed this new category in the taxonomy of Schop et al. \cite{schopf2023exploring} in Fig.\ref{fig:nlptaxonomy} in the Linguistics and Cognitive NLP category. However, it cannot be considered isolated, as all highlighted fields contribute to this field. In the following, we want to investigate further the term ``Computational Rhetoric'' and its actual meaning.








==> tex/glossary.tex <==
\newglossaryentry{anagram}
{       name= anagram,
        description={Word rearrangement by word or syllable rearrangement (permutation) used for puns or pseudonyms, also use of another name in place of one's own~\cite{Berner2011}}
}
\newglossaryentry{anaphora}
{       name= anaphora,
        description={Repetition of the initial word in successive sentences or lines~\cite{Berner2011}}
}

\newglossaryentry{alliteration}
{
        name=alliteration,
        description={The same sound of the stressed syllables within a word group \cite{gluck2016metzler}}
}

\newglossaryentry{antimetabole}
{       name= antimetabole,
        description={Repetition of words in two sentences of the same structure in reverse order (e.g., We do not live to eat, but we eat to live)~\cite{dudenAnti}}
}

\newglossaryentry{aphaeresis}
{       name= aphaeresis,
        description={Removal, disappearance of a vowel in the initial sound of a word~\cite{Berner2011}}
}

\newglossaryentry{apocope}
{       name= apocope,
        description={Truncation, omission of a letter at the end of a word~\cite{Berner2011}}
}

\newglossaryentry{apostrophe}
{       name= apostrophe,
        description={Turning away; a turning away from reality and turning toward invoking visionary figures or absentees as if they were present, in a broad sense also any ceremonial address~\cite{Berner2011}}
}

\newglossaryentry{archaism}
{       name= archaism,
        description={Antiquity; use of obsolete words or phrases, also called: antiquitas~\cite{Berner2011}}
}

\newglossaryentry{chiasmus}
{
        name=chiasmus,
        description={Crossing over of syntactically or semantically corresponding parts of sentences (``art is long, and short is our life'' \cite{Berner2011}}
}

\newglossaryentry{chiffre}
{       name= chiffre,
        description={Image or word compounds take on a meaning set by the author, regardless of their original meaning; sign whose content is enigmatic and cannot be grasped, or can only be grasped, by the author or from the context; the Schülerduden gives *one* example: "flight" as a cipher for the as a departure into the unknown [...] "city" as a cipher for hopelessness in some expressionist poets, occasionally the cipher is also called an absolute metaphor~\cite{Berner2011}}
}

\newglossaryentry{chroma}
{       name= chroma,
        description={TODO}
}

\newglossaryentry{climax}
{       name= climax,
        description={Ladder, staircase; an increase of at least three parts from the weaker to the stronger expression, sometimes also called gradation, but in German it coincides with the grammatical adjective increase (comparison), and only in connection with this it can also become a climax~\cite{Berner2011}}
}

\newglossaryentry{elision}
{       name= elision,
        description={Expulsion of a final unstressed vowel~\cite{Berner2011}}
}

\newglossaryentry{epanaphora}
{       name= epanaphora,
        description={Another word for \gls{anaphora}}
}

\newglossaryentry{epenthesis}
{       name= epenthesis,
        description={Insertion of a sound usually for phonological reasons~\cite{gluck2016metzler}}
}

\newglossaryentry{epiphora}
{       name= epiphora,
        description={Reversal of anaphora, repetition of one or more words at the end of a sentence or verse~\cite{Berner2011}}
}

\newglossaryentry{gradatio}
{       name= gradatio,
        description={Gradual increase; sequence of stages, generic term for climax and anticlimax~\cite{Berner2011}}
}
\newglossaryentry{homoioarcton}
{       name= homoioarcton,
        description={Figure of speech in which the beginnings of two consecutive words are the same or similar~\cite{dudenHomoe}}
}

\newglossaryentry{incrementum}
{       name= incrementum,
        description={A series of words in the same domain where subsequent words mark an increase on a semantic scale~\cite{o2018arguments}}
}

\newglossaryentry{irony}
{       name= irony,
        description={Pretense, mockery; feigned ignorance, pretense; the opposite of what is said is meant, irony is context-dependent or arises from the contradiction to the person and situation of the person using it; it has an alibi function, if one thereby hides one's true opinion, then the contradiction to the context is only recognizable to insiders; however, it can also have a mocking and aggressive character, if one presents the value judgment corresponding to the listener's expectation in the form of ironic praise~\cite{Berner2011}}
}

\newglossaryentry{malapropism}
{       name= malapropism,
        description={[deliberately] incorrect choice of words, in which a word is replaced by one that is phonologically similar but semantically (very) different~\cite{dudenMal}}
}

\newglossaryentry{melioration}
{       name= melioration,
        description={Improvement. Example: sweetheart instead of spouse~\cite{Berner2011}}
}

\newglossaryentry{metaphor}
{       name= metaphor,
        description={To transfer to something; a figure of figurative speech, the use of a word not in its proper (lexical) but (non-proper) transferred sense; the transfer of a word into a contextual image while retaining a similarity. A metaphor is a word in a context by which it is determined to mean something other than it means~\cite{Berner2011}}
}

\newglossaryentry{metathesis}
{       name= metathesis,
        description={(``Rearrangement''. Also: transposition) Sound change consisting in the rearrangement of a sound or interchange of sounds within words. Also common in loan words and in children's speech. The interchange may occur (a) within a syllable or (b) from one syllable to another~\cite{gluck2016metzler}}
}

\newglossaryentry{morphologic}
{       name= morphologic,
        description={TODO}
}

\newglossaryentry{parallelism}
{       name= parallelism,
        description={Repetition of the same syntactic construction in at least two or three successive clauses, often associated with an intensification or growing members~\cite{Berner2011}}
}

\newglossaryentry{pejoration}
{       name= pejoration,
        description={In linguistics, a word whose meaning has deteriorated in the course of development~\cite{Berner2011}}
}

\newglossaryentry{periphrasis}
{       name= periphrasis,
        description={Circumscription by characterizing activities, properties, or effects, also used to avoid a commonplace expression or to disguise naming; depending on the expressive intent, the periphrasis always captures only \textbf{one} characteristic among many: Rome - the eternal city, the capital of Italy, the city of the seven hills~\cite{Berner2011}}
}

\newglossaryentry{pragmatic}
{       name= pragmatic,
        description={TODO}
}

\newglossaryentry{prosthesis}
{       name= prosthesis,
        description={Addition of a sound at the beginning of a word [...]~\cite{gluck2016metzler}}
}

\newglossaryentry{rhetorical_question}
{       name= rhetorical question,
        description={ Rhetorical figure (of thought); question to which the speaker does not expect an answer and in which he or she dresses a request or statement. When the speaker wants to be particularly forceful and emotional~\cite{gluck2016metzler}},
        plural={rhetorical questions},
}

\newglossaryentry{semantic}
{       name= semantic,
        description={TODO}
}

\newglossaryentry{syllepsis}
{       name= syllepsis,
        description={Form of syntactic shortening in which a predicate verb is related to two or more grammatically identical but semantically different parts of a sentence, also called oblique parenthesis, since disparate things are brought together in a formal but stylistically oblique parenthesis~\cite{Berner2011}}
}

\newglossaryentry{symploce}
{       name= symploce,
        description={In a narrower sense the combination of \gls{anaphora} and \gls{epiphora}, in a broader sense also the connection of several repeated figures within a syntactic unit~\cite{Berner2011}}
}

\newglossaryentry{syncope}
{       name= syncope,
        description={Abbreviation; omission of a short vowel inside a word~\cite{Berner2011}}
}




\newacronym{RNG}{RNG}{Random Number Generator}
\newacronym{VNE}{VNE}{Virtual Network Embedding}
\newacronym{VNR}{VNR}{Virtual Network Request}
\newacronym{VN}{VN}{\gls{Virtual Network}}
\newacronym{VM}{VM}{Virtual Machine}
\newacronym{SN}{SN}{\gls{Substrate Network}}
\newacronym{NV}{NV}{Network Virtualization}
\newacronym{DES}{DES}{Discrete Event Simulator}
\newacronym{GUI}{GUI}{Graphical User Interface}
\newacronym{SUT}{SUT}{System Under Test}
\newacronym{NIDS}{NIDS}{Network Intrusion Detection System}
\newacronym{raid}{RAID}{Redundant Array of Independent Disks}
\newacronym{XML}{XML}{Extensible Markup Language}
\newacronym{XSD}{XSD}{\gls{XML} Schema Definition}
\newacronym{API}{API}{Application Programming Interface}
\newacronym{NWM}{NWM}{Network Weight Matrix}
\newacronym{ARS}{ARS}{Approximate Resource Scarcity}
\newacronym{GLPK}{GLPK}{GNU Linear Programming Kit}
\newacronym{OS}{OS}{Operating System}
\newacronym{VMI}{VMI}{Virtual Machine Introspection}
\newacronym{TPM}{TPM}{Trusted Platform Module}
\newacronym{IaaS}{IaaS}{Infrastructure as a Service}
\newacronym{TH}{TH}{Trusted Hardware}
\newacronym{CDL}{CDL}{Cross-domain Link}
\newacronym{SLA}{SLA}{Service-level-agreement}
